Energy-efficient operation of neural operators for virtual sensing

Virtual sensing repeatedly reconstructs physical fields from changing observations, often on a fixed geometry. We investigate how shared spatial computation reduces the energy of these updates while retaining the selected checkpoint and its evaluated predictions. In a heat-exchanger service, standard compiler freezing and explicit trunk reuse give similar operating energy reductions relative to graph replay: approximately 1% at one request per second and 20% at forty requests per second. In 15 W mode with fixed clocks, reuse with graph replay completes the same request sequence with 22.0 to 22.5% less energy than eager execution, including preparation and waiting. DeepONet and Fourier neural operator (FNO) controls distinguish the effects of reusable arithmetic and launch overhead. Preparation, artifact construction, and worker replacement add costs outside repeated inference. These results connect operator structure to operating energy and show how update frequency and execution lifetime govern the benefit of computation reuse in physical-field virtual sensing.

==> latexmkrc <==
$pdf_mode = 1;
@default_files = ('full.tex');

# Build current SI labels when main.tex is selected as the main document.
if (!$ENV{'OPCERT_BUILDING_SI'} &&
    grep { /(?:^|[\\\/])main(?:\.tex)?$/ } @ARGV) {
    local $ENV{'OPCERT_BUILDING_SI'} = 1;
    my $status = system('latexmk', '-cd', '-pdf',
                        '-interaction=nonstopmode', '-halt-on-error',
                        '-outdir=.', '-jobname=si_main', 'si/si_main.tex');
    die "Cannot build SI cross-references\n" if $status != 0;
}


==> sections/extended_table1.tex <==
\begin{table}[p]
\centering\small
\caption{\textbf{Mechanisms address distinct parts of the execution contract.}
$\bullet$, an explicit role in the specified mechanism; $\circ$, conditional on the chosen implementation or integration; --, not supplied by that mechanism alone. The final column records evaluation in this study, not comparative superiority. A retained historical target is distinct from the repeatable output selected by a new execution.}
\label{tab:coverage}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.55}
\begin{tabular}{@{}p{.30\linewidth}*{6}{>{\centering\arraybackslash}p{.095\linewidth}}@{}}
\toprule
Mechanism & Historical target & Arithmetic constraints & Retained resources & Execution change & Recovery protocol & Evaluated here \\
\midrule
Determinism controls & -- & $\bullet$ & -- & $\circ$ & -- & $\bullet$ \\
Fixed TensorRT engine & -- & $\bullet$ & $\circ$ & $\bullet$ & -- & -- \\
Reproducible CUB reduction & -- & $\bullet$ & -- & $\bullet$ & -- & -- \\
CUDA graph execution & -- & $\circ$ & $\circ$ & $\bullet$ & -- & $\bullet$ \\
Dedicated reusable pool & -- & -- & $\bullet$ & $\circ$ & -- & $\bullet$ \\
Fixed-query trunk reuse & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ & -- & $\bullet$ \\
Reference-qualified service & $\bullet$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ \\
\bottomrule
\end{tabular}
\vspace{1em}
\begin{minipage}{.96\linewidth}\footnotesize
\textbf{Scope of the columns.} ``Historical target'' means an independently retained output, not a captured plan or engine. ``Arithmetic constraints'' means restricting or retaining a numerical realisation; it does not imply a unique answer across environments. ``Retained resources'' denotes explicit persistent execution storage. ``Recovery protocol'' requires retirement and requalification against the original target, rather than mere continuation.

\medskip
\textbf{Documented alternatives.} TensorRT specifies the output of a built engine within its supported environment, with documented exceptions \citep{nvidia2026tensorrtdeterminism}. CUB supports selected deterministic reductions, including supported run-to-run or GPU-to-GPU modes \citep{nvidia2026cccldeterminism}. Neither was evaluated here as a complete-model historical-reference or paced-service baseline.

\medskip
\textbf{Evaluated mechanisms.} Graph capture can preserve a chosen operation sequence but does not specify an independent historical answer. The prepared graph paths own persistent storage. A dedicated eager pool retains reusable storage without replay (Fig.~\ref{fig:history}). Trunk reuse preserves a reference-computed intermediate only under its declared dependency and numerical conditions (Fig.~\ref{fig:physical}). The service combines qualification, monitored-condition checks and requalification; returned-output equality is audited after the measured blocks (Fig.~\ref{fig:service}). Determinism controls are tested separately in Supplementary Table~17.
\end{minipage}
\end{table}


==> sections/table1.tex <==
\begin{table}[t]\centering\footnotesize\setlength{\tabcolsep}{3pt}
\caption{\textbf{Prospective memory-cap tests on eight held-out releases.} The empirical scale $P=A_{\mathrm{peak}}+W_{\max}$ combines peak allocation with the largest executed workspace in one uncapped logged forward on the RTX~5060~Ti. $P$ and the initial test caps were recorded before each prospective round. All eight releases completed at nominal $1.10P$ (caps rounded to $0.0001$\,GiB) with zero unequal elements and zero allocator refusals; the calibration control was at $1.08P$. The refusal and unequal-output columns give the largest tested caps with those outcomes, not exact transition boundaries. Parentheses give allocator refusal counts. $^\dagger$Additional cap tested after its prospective round. The original joint predictions succeeded for 2/4 checkpoints in round one and 1/4 in round two. Engine landings are detailed in Extended Data Fig.~3.}\label{tab:prediction}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrlll@{}}
\toprule
Checkpoint task & \shortstack{$A_{\mathrm{peak}}$\\(GiB)} & \shortstack{$W_{\max}$\\(MiB)} & \shortstack{$P$\\(GiB)} & \shortstack{Refusal cap\\(count)} & \shortstack{Unequal-output\\cap} & \shortstack{Unequal elements\\/ total}\\
\midrule
\multicolumn{7}{@{}l}{\textit{Calibration}}\\
Rayleigh--Bénard & 0.1734 & 59.6 & 0.2316 & $0.86P$ (16) & $0.86P$ & 261{,}675 / 262{,}144\\
\midrule
\multicolumn{7}{@{}l}{\textit{Prospective round one}}\\
Active matter & 0.1809 & 36.2 & 0.2162 & $0.90P$ (11) & $0.90P$ & 720{,}878 / 720{,}896\\
Gray--Scott & 0.0959 & 23.3 & 0.1186 & $0.90P$ (31) & $0.90P$ & 31{,}277 / 32{,}768\\
Shear flow & 0.2805 & 72.2 & 0.3510 & $0.90P$ (9) & $0.85P$$^\dagger$ & 524{,}269 / 524{,}288\\
Helmholtz & 0.4881 & 144.2 & 0.6289 & $0.83P$$^\dagger$ (9) & $0.76P$$^\dagger$ & 522{,}704 / 524{,}288\\
\midrule
\multicolumn{7}{@{}l}{\textit{Prospective round two}}\\
Acoustic maze & 0.1729 & 36.2 & 0.2082 & $0.90P$ (11) & $0.90P$ & 196{,}600 / 196{,}608\\
Planetary shallow water & 0.2786 & 72.2 & 0.3491 & $0.90P$ (9) & $0.85P$$^\dagger$ & 393{,}186 / 393{,}216\\
Viscoelastic instability & 0.5106 & 144.2 & 0.6514 & $0.90P$ (4) & $0.75P$ & 2{,}096{,}300 / 2{,}097{,}152\\
Turbulent radiative layer & 0.1483 & 27.2 & 0.1748 & $0.90P$ (11) & $0.90P$ & 196{,}594 / 196{,}608\\
\bottomrule
\end{tabular*}
\end{table}

